Unsupervised Active Visual Search with Monte Carlo planning under Uncertain Detections

We propose a solution for Active Visual Search of objects in an environment, whose 2D floor map is the only known information. Our solution has three key features that make it more plausible and robust to detector failures compared to state-of-the-art methods: (i) it is unsupervised as it does not need any training sessions. (ii) During the exploration, a probability distribution on the 2D floor map is updated according to an intuitive mechanism, while an improved belief update increases the effectiveness of the agent's exploration. (iii) We incorporate the awareness that an object detector may fail into the aforementioned probability modelling by exploiting the success statistics of a specific detector. Our solution is dubbed POMP-BE-PD (Pomcp-based Online Motion Planning with Belief by Exploration and Probabilistic Detection). It uses the current pose of an agent and an RGB-D observation to learn an optimal search policy, exploiting a POMDP solved by a Monte-Carlo planning approach. On the Active Vision Database benchmark, we increase the average success rate over all the environments by a significant 35% while decreasing the average path length by 4% with respect to competing methods. Thus, our results are state-of-the-art, even without using any training procedure.

==> abstract_uncut.tex <==
%%%%%%%%%%%%%%%%%%%% NEW ABSTRACT - MARCO %%%%%%%%%%%%
In this paper we propose a solution for Active Visual Search of objects in an environment, whose 2D floor map is the only known information. Our solution has three key features:
\textit{(i)} it is unsupervised as it does not need any training session, making it more practical to use. In fact, our agent makes decisions on the next moves by iterating over the scenario at hand, exploring the environment and searching for the object at the same time.
\textit{(ii)} During the exploration, a probability distribution on the 2D floor map is updated according to an intuitive mechanism: if the target object is not found in a certain location, it must be elsewhere inside the environment. On top of that, we increase the effectiveness of the agent's exploration with an improved belief update.
% \textit{(ii)} During the exploration, a probability distribution on the 2D floor map is updated according to an intuitive mechanism: if the target object is not found in a certain location, the remaining locations will become more important to explore. This translates into an updated belief distribution that makes the search faster.
% \textit{(iii)}~Our solution incorporates the awareness that an object detector may fail, exploiting the success statistics of a specific detector within the reasoning. This makes the approach more plausible, compared to assuming an infallible detector, as occurs in the state of the art.
% %
\textit{(iii)}~Our solution incorporates the awareness that an object detector may fail into the aforementioned probability modelling by exploiting the success statistics of a specific detector. These three key features make the approach more plausible in motion planning and more robust to detector failures compared to the state-of-the-art methods.
%
Our solution is dubbed as \methname~(Pomcp-based Online Motion Planning with Belief by Exploration and Probabilistic Detection). It takes the current pose of an agent (\eg a robot) and RGB-D observation as input and learns an optimal search policy for Active Visual Search, exploiting a Partially Observable Markov Decision Process solved by a Monte-Carlo planning approach. 
%As input, it uses the current pose of an agent (\eg a robot) and an RGB-D frame. 
%
We validate our approach on the publicly available Active Vision Database benchmark, increasing the average success rate over all the environments by a significant 35$\%$ while decreasing the average path length by 4$\%$ with respect to competing methods.
% As a consequence, our results are \ftaioli{close to the }state-of-the-art, even without using any training procedure.
Thus, our results are state-of-the-art, even without using any training procedure.
